A Roadmap to Domain Knowledge Integration in Machine Learning

Many machine learning algorithms have been developed in recent years to enhance the performance of a model in different aspects of artificial intelligence. But the problem persists due to inadequate data and resources. Integrating knowledge in a machine learning model can help to overcome these obstacles up to a certain degree. Incorporating knowledge is a complex task though because of various forms of knowledge representation. In this paper, we will give a brief overview of these different forms of knowledge integration and their performance in certain machine learning tasks.

==> save.tex <==
\begin{thebibliography}{00}
\bibitem{b1} G. Marcus, “Innateness, alphazero, and artificial intelligence”, CoRR, vol. abs/1801.05667, 2018.
\bibitem{b2}  G.P. Goodwin and  P.N. Johnson-Laird, "Reasoning about relations", Psychol, Rev. 112, 468–493, 2005.

\bibitem{b3}  Halford G.S, Wilson WH, Phillips S  (1998). "Processing capacity defined by relational
complexity: Implications for comparative, developmental, and
cognitive psychology, Behav. Brain Sci., 21, 803–831.

\bibitem{b4} D. Ganguly, D. Roy, M. Mitra and G.F.J. Jones, "Word Embedding Based Generalized Language Model for Information Retrieval", Proceedings of the 38th International ACM SIGIR Conference on Research and Development in Information Retrieval, Pages 795–798, 2005.

\bibitem{b5} Z. Chi. "Statistical properties of probabilistic context-free grammars", Computational Linguistics,  25.1, 131-160, 1999.

\bibitem{b6} M. Richardson and P. Domingos. ""Markov logic networks", Machine learning, 62.1-2, 107-136, 2006.
\bibitem{b7}H. Sun, B. Dhingra, M. Zaheer, K. Mazaitis, R. Salakhutdinov and W. W. Cohen  (2018), "Open domain question answering using early fusion of knowledge bases and text.", arXiv preprint arXiv:1809.00782.

\bibitem{b8} M. Diligenti, S. Roychowdhury, and M. Gori, "Integrating prior knowledge into deep learning.", 16th IEEE International Conference on Machine Learning and Applications (ICMLA), IEEE, 2017.

\bibitem{b9}N. Muralidhar, M. R. Islam, M. Marwah, A. Karpatne and N. Ramakrishnan, "Incorporating prior domain knowledge into deep neural networks", 2018 IEEE International Conference on Big Data (Big Data) (pp. 36-45). IEEE, 2018.

\bibitem{b10} Z. Hu, X. Ma, Z. Liu, E. Hovy and E. Xing, "Harnessing deep neural networks with logic rules.", arXiv preprint arXiv:1603.06318, 2016.

\bibitem{b11} G. Hinton, O. Vinyals, and J. Dean, "Distilling the knowledge in a neural network.", arXiv preprint arXiv:1503.02531, 2015.

\bibitem{b12}Z. Hu, Z. Yang, R. Salakhutdinov, L.Qin, X. Liang, H. Dong and E. P. Xing, "Deep generative models with learnable knowledge constraints", Advances in Neural Information Processing Systems (pp. 10501-10512), 2018.

\bibitem{b13} S. Radovanović, B. Delibašić, M. Jovanović, M. Vukićević, and M. Suknović, "Framework for integration of domain knowledge into logistic regression.", Proceedings of the 8th International Conference on Web Intelligence, Mining and Semantics (WIMS ’18), Association for Computing Machinery, New York, NY, USA, Article 24, 1–8, 2018.

\bibitem{b14} J. Xu, , Z. Zhang, T. Friedman, Y. Liang, G. V. D. Broeck, "A semantic loss function for deep learning with symbolic knowledge.", arXiv preprint arXiv:1711.11157, 2017.

\bibitem{b15}C. J. Shallue, and A. Vanderburg, "Identifying Exoplanets with Deep Learning: A Five-planet Resonant Chain around Kepler-80 and an Eighth Planet around Kepler-90", The Astronomical Journal, volume 155, number 2, 2018. 

\bibitem{b16} M. Ansdell, Y. Ioannou, H. P. Osborn, M. Sasdelli, J. C. Smith, D. Caldwell, J. M. Jenkins, C. Räissi, and D. Angerhausen, "Scientific Domain Knowledge Improves Exoplanet Transit Classification with Deep Learning.", The Astrophysical Journal Letters 869, no. 1 (2018): L7, 2018.

\bibitem{b17} R. Stewart, and S. Ermon, "Label-free supervision of neural networks with physics and domain knowledge." , Thirty-First AAAI Conference on Artificial Intelligence. 2017.

\bibitem{b18}Y. Xie, Z. Xu , M. S. Kankanhalli, K. S. Meel, and H. Soh, "Embedding Symbolic Knowledge into Deep Networks.", arXiv preprint arXiv:1909.01161, 2019.

\bibitem{b19}N. Pitelis, C. Russell, and L. Agapito, "Semi-supervised
learning using an unsupervised atlas.", ECML-PKDD,
pp. 565–580. Springer, 2014.

\bibitem{b20} D. P. Kingma, S. Mohamed, D. Jimenez Rezende, and
M. Welling, "Semi-supervised learning with deep generative
models." , NIPS, pp. 3581–3589. Curran Associates, Inc., 2014.

\bibitem{b21}T. Miyato, S.I. Maeda, M. Koyama, K. Nakae, and
S. Ishii, "Distributional smoothing with virtual adversarial
training." In ICLR, 2016.

\bibitem{b22}A. Rasmus, M. Berglund,  M. Honkala, H. Valpola, and
T. Raiko,  "Semi-supervised learning with ladder networks.", NIPS, 2015.

\bibitem{b23}L. Ma, Q. Sun, S. Georgoulis, L. Van Gool, B. Schiele, and M. Fritz. "Disentangled person image generation", CVPR, 2018.

\bibitem{b24}A. Pumarola, A. Agudo, A. Sanfeliu, and F. Moreno-Noguer, "Unsupervised person image synthesis in
arbitrary poses.", CVPR, 2018.
\bibitem{b25}L. Ma, X. Jia, Q. Sun, B. Schiele, T. Tuytelaars, and L. Van Gool, "Pose guided person image generation.", NIPS, pages 405–415, 2017.

\bibitem{b26}A. Darwiche, "Decomposable negation normal form." Journal of the ACM (JACM) 48.4 (2001): 608-647.

\bibitem{b27}L. Yao, M. Chengsheng, and L. Yuan, "KG-BERT: BERT for knowledge graph completion",  arXiv preprint arXiv:1909.03193 (2019).

\bibitem{b28}T. Mikolov, K. Chen, G. Corrado, and J. Dean, "Efficient estimation of word
representations in vector space", arXiv preprint
arXiv:1301.3781, 2013.


\bibitem{b29}Y. Sun, S. Wang, Y. Li, S. Feng, X. Chen, H. Zhang, X. Tian, D. Zhu, H. Tian, and H. Wu, Ernie: Enhanced representation through knowledge integration. arXiv preprint arXiv:1904.09223, 2019.


\bibitem{b30}Zhang, X. H. Zhengyan, L. Zhiyuan, J. Xin, S. Maosong, and L. Qun, "ERNIE: Enhanced language representation with informative entities.", arXiv preprint arXiv:1905.07129 (2019).


\end{thebibliography}
